Using Source Code Metrics for Predicting Metamorphic Relations at Method Level

Metamorphic testing (TM) examines the relations between inputs and outputs of test runs. These relations are known as metamorphic relations (MR). Currently, MRs are handpicked and require in-depth knowledge of the System Under Test (SUT), as well as its problem domain. As a result, the identification and selection of high-quality MRs is a challenge. \citeauthor{PMR1} suggested the Predicting Metamorphic Relations (PMR) approach for automatic prediction of applicable MRs picked from a predefined list. PMR is based on a Support Vector Machine (SVM) model using features derived from the Control Flow Graphs (CFGs) of 100 Java methods. The original study of \citeauthor{PMR1} showed encouraging results, but developing classification models from CFG-related features is costly. In this paper, we aim at developing a PMR approach that is less costly without losing performance. We complement the original PMR approach by considering other than CFG-related features. We define 21 features that can be directly extracted from source code and build several classifiers, including SVM models. Our results indicate that using the original CFG-based method-level features, in particular for a SVM with random walk kernel (RWK), achieve better predictions in terms of AUC-ROC for most of the candidate MRs than our models. However, for one of the candidate MRs, using source code features achieved the best AUC-ROC result (greater than 0.8).

==> RQ1-V2.tex <==
\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting ADD}
\label{tbl:RQ1_ADD}
\centering
\resizebox{8.9cm}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll}
    \toprule
    \multirow{2}{*}{\textbf{Clas$^\star$}}
    &\multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1 score}} & \multicolumn{2}{c}{\textbf{AUC-ROC}} \\
    
    & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ \\
 
    \midrule
    RF	&	\textbf{0.886}	&	0.002	&	0.767	&	-0.003	&	\textbf{0.971}	&	-0.002	&	0.830	&	0.006	&	\textbf{0.886}	&	0.296	\\
    DT	&	0.800	&	0.120	&	0.812	&	0.087	&	0.833	&	0.167	&	0.727	&	0.071	&	0.816	&	0.118	\\
    GNB	&	0.833	&	0.107	&	\textbf{0.914}	&	0.219	&	0.833	&	0.107	&	0.823	&	0.054	&	0.875	&	0.208	\\
    SVM	&	0.803	&	0.183	&	0.833	&	0.158	&	0.838	&	0.218	&	\textbf{0.835}	&	0.176	&	0.833	&	0.161	\\
    LG	&	0.800	&	0.120	&	0.807	&	0.114	&	0.833	&	0.143	&	0.833	&	0.143	&	0.800	&	0.125	\\

	\bottomrule
	\multicolumn{10}{l}{$^\star$Classifier, $^\pm$diff (Feat$_{12}$ - Feat$_{20}$)}
	\end{tabular}}
\end{table}

%EXC

\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting EXC}
\label{tbl:RQ1_EXC}
\centering
\resizebox{8.9cm}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll}
    \toprule
    \multirow{2}{*}{\textbf{Clas$^\star$}}
    &\multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1 score}} & \multicolumn{2}{c}{\textbf{AUC-ROC}} \\
    
    & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ \\
 
    \midrule
    RF	&	\textbf{0.800}	&	0.150	&	\textbf{0.866}	&	0.252	&	\textbf{1.000}	&	0.334	&	0.800	&	0.134	&	\textbf{0.833}	&	0.167	\\
    DT	&	0.750	&	0.180	&	0.844	&	0.149	&	0.667	&	0.135	&	0.602	&	0.102	&	0.667	&	0.131	\\
    GNB	&	0.712	&	0.045	&	0.800	&	0.134	&	0.667	&	0.133	&	0.667	&	0.206	&	0.619	&	0.048	\\
    SVM	&	0.704	&	0.064	&	0.733	&	0.066	&	0.667	&	0.137	&	\textbf{0.857}	&	0.295	&	0.694	&	0.121	\\
    LG	&	0.657	&	-0.010	&	0.844	&	0.219	&	0.665	&	0.075	&	0.671	&	0.100	&	0.696	&	0.173	\\

	\bottomrule
	\multicolumn{10}{l}{$^\star$Classifier, $^\pm$diff (Feat$_{12}$ - Feat$_{20}$)}
	\end{tabular}}
\end{table}

% INC
\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting INC}
\label{tbl:RQ1_INC}
\centering
\resizebox{8.9cm}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll}
    \toprule
    \multirow{2}{*}{\textbf{Clas$^\star$}}
    &\multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1 score}} & \multicolumn{2}{c}{\textbf{AUC-ROC}} \\
    
    & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ \\
 
    \midrule
    RF	&	\textbf{0.900}	&	0.270	&	\textbf{0.889}	&	0.237	&	\textbf{0.890}	&	0.224	&	\textbf{0.888}	&	0.161	&	0.717	&	0.023	\\
    DT	&	0.750	&	0.138	&	0.616	&	0.100	&	0.596	&	0.263	&	0.589	&	0.152	&	0.605	&	0.082	\\
    GNB	&	0.705	&	0.037	&	0.862	&	0.258	&	0.667	&	0.080	&	0.667	&	0.125	&	0.681	&	0.171	\\
    SVM	&	0.802	&	0.192	&	0.806	&	0.139	&	0.645	&	0.111	&	0.667	&	0.219	&	\textbf{0.761}	&	0.213	\\
    LG	&	0.701	&	0.088	&	0.695	&	0.094	&	0.668	&	0.071	&	0.571	&	0.238	&	0.690	&	0.261	\\

	\bottomrule
	\multicolumn{10}{l}{$^\star$Classifier, $^\pm$diff (Feat$_{12}$ - Feat$_{20}$)}
	\end{tabular}}
\end{table}


% MUL
\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting MUL}
\label{tbl:RQ1_MUL}
\centering
\resizebox{8.9cm}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll}
    \toprule
    \multirow{2}{*}{\textbf{Clas$^\star$}}
    &\multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1 score}} & \multicolumn{2}{c}{\textbf{AUC-ROC}} \\
    
    & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ \\
 
    \midrule
    RF	&	0.800	&	0.150	&	0.853	&	0.196	&	\textbf{1.000}	&	0.177	&	\textbf{0.875}	&	0.127	&	0.762	&	0.184	\\
    DT	&	0.703	&	0.083	&	0.802	&	0.107	&	0.833	&	0.011	&	0.833	&	0.114	&	0.791	&	0.140	\\
    GNB	&	0.700	&	0.040	&	0.834	&	0.159	&	0.940	&	0.083	&	0.823	&	0.041	&	0.625	&	0.101	\\
    SVM	&	\textbf{0.804}	&	0.194	&	0.850	&	0.117	&	0.857	&	0.024	&	0.857	&	0.231	&	0.761	&	0.071	\\
    LG	&	0.801	&	0.121	&	\textbf{0.875}	&	0.206	&	0.857	&	0.034	&	\textbf{0.875}	&	0.116	&	\textbf{0.833}	&	0.083	\\

	\bottomrule
	\multicolumn{10}{l}{$^\star$Classifier, $^\pm$diff (Feat$_{12}$ - Feat$_{20}$)}
	\end{tabular}}
\end{table}

% PER
\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting PER}
\label{tbl:RQ1_PER}
\centering
\resizebox{8.9cm}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll}
    \toprule
    \multirow{2}{*}{\textbf{Clas$^\star$}}
    &\multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1 score}} & \multicolumn{2}{c}{\textbf{AUC-ROC}} \\
    
    & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ \\
 
    \midrule
    RF	&	0.810	&	0.190	&	0.814	&	0.189	&	\textbf{0.712}	&	0.146	&	0.789	&	0.127	&	0.747	&	0.000	\\
    DT	&	0.750	&	0.084	&	\textbf{0.914}	&	0.137	&	0.775	&	0.109	&	\textbf{0.857}	&	0.281	&	\textbf{0.857}	&	0.096	\\
    GNB	&	0.700	&	0.155	&	0.828	&	0.206	&	0.666	&	0.333	&	0.727	&	0.277	&	0.642	&	0.076	\\
    SVM	&	\textbf{0.910}	&	0.070	&	0.875	&	0.076	&	0.750	&	0.083	&	0.729	&	0.062	&	0.825	&	0.064	\\
    LG	&	0.830	&	0.130	&	0.822	&	0.039	&	0.709	&	0.042	&	0.750	&	0.060	&	0.795	&	0.101	\\

	\bottomrule
	\multicolumn{10}{l}{$^\star$Classifier, $^\pm$diff (Feat$_{12}$ - Feat$_{20}$)}
	\end{tabular}}
\end{table}

% INV
\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting INV}
\label{tbl:RQ1_INV}
\centering
\resizebox{8.9cm}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll}
    \toprule
    \multirow{2}{*}{\textbf{Clas$^\star$}}
    &\multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1 score}} & \multicolumn{2}{c}{\textbf{AUC-ROC}} \\
    
    & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ \\
 
    \midrule
    RF	&	0.702	&	0.094	&	0.833	&	0.158	&	\textbf{0.857}	&	0.138	&	0.800	&	0.049	&	0.625	&	-0.015	\\
    DT	&	0.800	&	0.200	&	\textbf{0.844}	&	0.282	&	\textbf{0.857}	&	0.190	&	0.714	&	0.047	&	0.667	&	0.126	\\
    GNB	&	0.701	&	0.081	&	0.833	&	0.349	&	\textbf{0.857}	&	0.197	&	0.823	&	0.073	&	0.625	&	0.114	\\
    SVM	&	0.802	&	0.052	&	\textbf{0.844}	&	0.152	&	0.833	&	0.069	&	\textbf{0.857}	&	0.088	&	\textbf{0.857}	&	0.190	\\
    LG	&	\textbf{0.860}	&	0.184	&	0.761	&	0.066	&	\textbf{0.857}	&	0.126	&	\textbf{0.857}	&	0.181	&	0.762	&	0.095	\\

	\bottomrule
	\multicolumn{10}{l}{$^\star$Classifier, $^\pm$diff (Feat$_{12}$ - Feat$_{20}$)}
	\end{tabular}}
\end{table}

==> RQ1.tex <==
\begin{comment}
\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting ADD}
\label{tbl:RQ1_ADD}
\centering
	%\resizebox{18cm}{!}{
\begin{tabular}{l|l|l|l|l|l}
    \toprule
    \textbf{Classifier} &{\textbf{Accuracy}} & {\textbf{Precision}} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} \\	

    \midrule
    RF(12)	&\textbf{0.8859}&	\textbf{0.7695}	&	0.9709	    &	\textbf{0.8299}	&	0.8979	\\
    RF(20)	&	0.8841	    &	0.7667	        &	0.9726	    &	0.8235	&	\textbf{0.8981}	\\
    DT	&	0.8802	        &	0.7494	        &	\textbf{0.9834}	&	0.8343	&	0.8872	\\
    GNB	&	0.8533	        &	0.7675	        &	0.8665	    &	0.7819	&	0.8752	\\
    SVM	&	0.8491	        &	0.7667	        &	0.7505	    &	0.7209	&	0.8739	\\
    LG	&	0.8338	        &	0.7684	        &	0.8063	    &	0.7622	&	0.8497	\\

	\bottomrule
	\end{tabular}%}
\end{table}
\end{comment}


\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting ADD}
\label{tbl:RQ1_ADD}
\centering
\resizebox{8.8cm}{!}{
\begin{tabular}{l|ll|ll|ll|ll|ll}
    \toprule
    \multirow{2}{*}{\textbf{Clas$^\star$}}
    &\multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1 score}} & \multicolumn{2}{c}{\textbf{AUROC}} \\
    
    & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ & Feat$_{12}$ & diff$^\pm$ \\
 
    \midrule
    RF	&\textbf{0.886}&    &	\textbf{0.7695}	&    &	0.9709	    &    &	\textbf{0.8299}	&    &	0.8979	\\
    DT	&	0.880	   &    &	0.7494	        &    &	\textbf{0.9834}	&    &	0.8343	&    &	0.8872	\\
    GNB	&	0.853      &    &	0.7675	        &    &	0.8665	    &    &	0.7819	&    &	0.8752	\\
    SVM	&	0.849      &    &	0.7667	        &    &	0.7505	    &    &	0.7209	&    &	0.8739	\\
    LG	&	0.834      &    &	0.7684	        &    &	0.8063	    &    &	0.7622	&    &	0.8497	\\

	\bottomrule
	\multicolumn{10}{l}{$^\star$Classifier, $^\pm$diff (Feat$_{12}$ - Feat$_{20}$)}
	\end{tabular}}
\end{table}


\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting MUL}
\label{tbl:RQ1_MUL}
\centering
	%\resizebox{18cm}{!}{
\begin{tabular}{l|l|l|l|l|l}
    \toprule
    \textbf{Classifier} &{\textbf{Accuracy}} & {\textbf{Precision}} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} \\	

    \midrule
    RF(12)	& 0.62  & 0.8214 & 0.62 & 0.7186 & 0.6523 \\
    RF(20)	& 0.6189  & 0.7874 & 0.6172 & 0.7086 & 0.6223	\\
    DT	&		\\
    GNB	&		\\
    SVM	&		\\
    LG	&	0.7847	& 0.6422 & 0.7275 & 0.6548 & 0.6150	\\

	\bottomrule
	\end{tabular}%}
\end{table}

\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting PER}
\label{tbl:RQ1_PER}
\centering
	%\resizebox{18cm}{!}{
\begin{tabular}{l|l|l|l|l|l}
    \toprule
    \textbf{Classifier} &{\textbf{Accuracy}} & {\textbf{Precision}} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} \\	

    \midrule
    RF(12)	&	\textbf{0.8466}	&	0.6554	&	0.7773	&	0.6879	&	\textbf{0.7779}	\\
    RF(20)	&	0.8442	        &	0.6545	&	0.7625	&	0.6764	&	0.777	\\
    DT	&	0.8397	            &	0.6407	&	\textbf{0.8032}	&	\textbf{0.6945}	&	0.7635	\\
    GNB	&	0.814	            &\textbf{0.657}5	&	0.7391	&	0.6695	&	0.7559	\\
    SVM	&	0.8038	            &	0.6294	&	0.6327	&	0.6012	&	0.7493	\\
    LG	&	0.8131	            &	0.651	&	0.6858	&	0.6454	&	0.7424	\\


	\bottomrule
	\end{tabular}%}
\end{table}


\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting INC}
\label{tbl:RQ1_INC}
\centering
	%\resizebox{18cm}{!}{
\begin{tabular}{l|l|l|l|l|l}
    \toprule
    \textbf{Classifier} &{\textbf{Accuracy}} & {\textbf{Precision}} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} \\	

    \midrule
    RF(12)	&		\\
    RF(20)	&	\\
    DT	&		\\
    GNB	&		\\
    SVM	&		\\
    LG	&		\\

	\bottomrule
	\end{tabular}%}
\end{table}


\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting EXC}
\label{tbl:RQ1_EXC}
\centering
	%\resizebox{18cm}{!}{
\begin{tabular}{l|l|l|l|l|l}
    \toprule
    \textbf{Classifier} &{\textbf{Accuracy}} & {\textbf{Precision}} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} \\	

    \midrule
    RF(12)	&		\\
    RF(20)	&	\\
    DT	&		\\
    GNB	&		\\
    SVM	&		\\
    LG	&		\\

	\bottomrule
	\end{tabular}%}
\end{table}



\begin{table}[!h]
\caption{PMR performance comparison of different classifiers when predicting INV}
\label{tbl:RQ1_INV}
\centering
	%\resizebox{18cm}{!}{
\begin{tabular}{l|l|l|l|l|l}
    \toprule
    \textbf{Classifier} &{\textbf{Accuracy}} & {\textbf{Precision}} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} \\	

    \midrule
    RF(12)	&		\\
    RF(20)	&	\\
    DT	&		\\
    GNB	&		\\
    SVM	&		\\
    LG	&		\\

	\bottomrule
	\end{tabular}%}
\end{table}
